An Interpretation of E-HA$^w$ inside HA$^w$

Higher Type Arithmetic (HA$^w$) is a first-order many-sorted theory. It is a conservative extension of Heyting Arithmetic obtained by extending the syntax of terms to all of System T: the objects of interest here are the functionals of higher types. While equality between natural numbers is specified by the axioms of Peano, how can equality between functionals be defined? From this question, different versions of HA$^w$ arise, such as an extensional version (E-HA$^w$) and an intentional version (I-HA$^w$). In this work, we will see how the study of partial equivalence relations leads us to design a translation by parametricity from E-HA$^w$ to HA$^w$.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{A. Ciaffaglione and C. Olarte (Eds.): Logical Frameworks\\
and Meta-Languages: Theory and Practice (LFMTP 2023)\\
EPTCS 396, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.396.5}{10.4204/EPTCS.396.5}}

